Detecting Anomalies in Software Execution Logs with Siamese Network

Logs are semi-structured text files that represent software's execution paths and states during its run-time. Therefore, detecting anomalies in software logs reflect anomalies in the software's execution path or state. So, it has become a notable concern in software engineering. We use LSTM like many prior works, and on top of LSTM, we propose a novel anomaly detection approach based on the Siamese network. This paper also provides an authentic validation of the approach on the Hadoop Distributed File System (HDFS) log dataset. To the best of our knowledge, the proposed approach outperforms other methods on the same dataset at the F1 score of 0.996, resulting in a new state-of-the-art performance on the dataset. Along with the primary method, we introduce a novel training pair generation algorithm that reduces generated training pairs by the factor of 3000 while maintaining the F1 score, merely a modest decay from 0.996 to 0.995. Additionally, we propose a hybrid model by combining the Siamese network with a traditional feedforward neural network to make end-to-end training possible, reducing engineering effort in setting up a deep-learning-based log anomaly detector. Furthermore, we examine our method's robustness to log evolutions by evaluating the model on synthetically evolved log sequences; we got the F1 score of 0.95 at the noise ratio of 20%. Finally, we dive deep into some of the side benefits of the Siamese network. Accordingly, we introduce a method of monitoring the evolutions of logs without label requirements at run-time. Additionally, we present a visualization technique that facilitates human administrations of log anomaly detection.

==> graphics/siamese_network_architecture_old.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Rounded Rect [id:dp5386810343511101] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 190; green, 233; blue, 160 }  ,fill opacity=1 ][line width=1.5]  (194,59.88) .. controls (194,46.48) and (204.86,35.63) .. (218.25,35.63) -- (337.05,35.63) .. controls (350.44,35.63) and (361.3,46.48) .. (361.3,59.88) -- (361.3,59.88) .. controls (361.3,73.27) and (350.44,84.13) .. (337.05,84.13) -- (218.25,84.13) .. controls (204.86,84.13) and (194,73.27) .. (194,59.88) -- cycle ;

%Straight Lines [id:da9702070763214259] 
\draw [line width=1.5]    (128.5,60.25) -- (190,59.9) ;
\draw [shift={(194,59.88)}, rotate = 539.6700000000001] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.07,-5.32) -- (0,0) -- (11.07,5.32) -- (7.35,0) -- cycle    ;
%Shape: Circle [id:dp6626219935087772] 
\draw  [fill={rgb, 255:red, 255; green, 246; blue, 138 }  ,fill opacity=1 ][line width=1.5]  (587,148) .. controls (587,134.19) and (598.19,123) .. (612,123) .. controls (625.81,123) and (637,134.19) .. (637,148) .. controls (637,161.81) and (625.81,173) .. (612,173) .. controls (598.19,173) and (587,161.81) .. (587,148) -- cycle ;

%Rounded Rect [id:dp28664661075314624] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 190; green, 233; blue, 160 }  ,fill opacity=1 ][line width=1.5]  (192,234.88) .. controls (192,221.48) and (202.86,210.63) .. (216.25,210.63) -- (335.05,210.63) .. controls (348.44,210.63) and (359.3,221.48) .. (359.3,234.88) -- (359.3,234.88) .. controls (359.3,248.27) and (348.44,259.13) .. (335.05,259.13) -- (216.25,259.13) .. controls (202.86,259.13) and (192,248.27) .. (192,234.88) -- cycle ;

%Straight Lines [id:da869241698880753] 
\draw [line width=1.5]    (126.5,235.5) -- (188,234.91) ;
\draw [shift={(192,234.88)}, rotate = 539.45] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.07,-5.32) -- (0,0) -- (11.07,5.32) -- (7.35,0) -- cycle    ;
%Curve Lines [id:da3265838127992584] 
\draw [line width=1.5]    (486.43,236) .. controls (601.36,236) and (611.52,192.59) .. (612.04,176.93) ;
\draw [shift={(612,173)}, rotate = 447.14] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.07,-5.32) -- (0,0) -- (11.07,5.32) -- (7.35,0) -- cycle    ;
%Rounded Rect [id:dp9698054751349445] 
\draw  [fill={rgb, 255:red, 172; green, 158; blue, 250 }  ,fill opacity=1 ][line width=1.5]  (688,148.5) .. controls (688,138.56) and (696.06,130.5) .. (706,130.5) -- (770.36,130.5) .. controls (780.3,130.5) and (788.36,138.56) .. (788.36,148.5) -- (788.36,148.5) .. controls (788.36,158.44) and (780.3,166.5) .. (770.36,166.5) -- (706,166.5) .. controls (696.06,166.5) and (688,158.44) .. (688,148.5) -- cycle ;

%Curve Lines [id:da6249121159046174] 
\draw [line width=1.5]    (485.43,59) .. controls (601.63,59.92) and (610.73,102.69) .. (611.82,119.15) ;
\draw [shift={(612,123)}, rotate = 267.61] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.07,-5.32) -- (0,0) -- (11.07,5.32) -- (7.35,0) -- cycle    ;
%Straight Lines [id:da1401459826986351] 
\draw [line width=1.5]    (637,148) -- (684,148.46) ;
\draw [shift={(688,148.5)}, rotate = 180.56] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.07,-5.32) -- (0,0) -- (11.07,5.32) -- (7.35,0) -- cycle    ;
%Straight Lines [id:da6532997273928633] 
\draw [line width=1.5]    (788.36,148.5) -- (835.36,148.96) ;
\draw [shift={(839.36,149)}, rotate = 180.56] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.07,-5.32) -- (0,0) -- (11.07,5.32) -- (7.35,0) -- cycle    ;
%Straight Lines [id:da0784554388542158] 
\draw [line width=1.5]    (361.3,59.88) -- (440,59.99) ;
\draw [shift={(444,60)}, rotate = 180.09] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.07,-5.32) -- (0,0) -- (11.07,5.32) -- (7.35,0) -- cycle    ;
%Straight Lines [id:da4792985730289756] 
\draw [line width=1.5]    (359.3,234.88) -- (441,234.99) ;
\draw [shift={(445,235)}, rotate = 180.08] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.07,-5.32) -- (0,0) -- (11.07,5.32) -- (7.35,0) -- cycle    ;

% Text Node
\draw (275.65,234.88) node  [font=\small] [align=left] {\begin{minipage}[lt]{78.76304pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{helvet}\selectfont Embedding Neural}\\{\fontfamily{helvet}\selectfont Network}
\end{center}

\end{minipage}};
% Text Node
\draw (738.18,148.5) node  [font=\small] [align=left] {Sigmoid};
% Text Node
\draw (612,148) node  [font=\small] [align=left] {Dot};
% Text Node
\draw (277.65,59.88) node  [font=\small] [align=left] {\begin{minipage}[lt]{78.76304pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{helvet}\selectfont Embedding Neural}\\{\fontfamily{helvet}\selectfont Network}
\end{center}

\end{minipage}};
% Text Node
\draw (126.5,60.25) node [anchor=east] [inner sep=0.75pt]    {$[ 1,\ 3,\ 7,\ 2,\ 3,\ 6]$};
% Text Node
\draw (124.5,235.5) node [anchor=east] [inner sep=0.75pt]    {$[ 1,\ 7,\ 3,\ 6,\ 2,\ 3]$};
% Text Node
\draw (484.43,236) node [anchor=east] [inner sep=0.75pt]  [font=\scriptsize]  {$\begin{bmatrix}
2.01\\
0.03\\
4.41\\
.\\
.\\
.\\
3.36
\end{bmatrix}$};
% Text Node
\draw (483.43,59) node [anchor=east] [inner sep=0.75pt]  [font=\scriptsize]  {$\begin{bmatrix}
1.12\\
0.01\\
3.46\\
.\\
.\\
.\\
4.97
\end{bmatrix}$};
% Text Node
\draw (841.36,149) node [anchor=west] [inner sep=0.75pt]    {$0.98$};


\end{tikzpicture}

